A geometrically converging dual method for distributed optimization over time-varying graphs

In this paper we consider a distributed convex optimization problem over time-varying undirected networks. We propose a dual method, primarily averaged network dual ascent (PANDA), that is proven to converge R-linearly to the optimal point given that the agents objective functions are strongly convex and have Lipschitz continuous gradients. Like dual decomposition, PANDA requires half the amount of variable exchanges per iterate of methods based on DIGing, and can provide with practical improved performance as empirically demonstrated.

==> bibliography <==
@article{decentralized_gradient,
author = {K.Yuan and Q. Ling and W. Yin},
title = {On the Convergence of Decentralized Gradient Descent},
journal = {SIAM Journal on Optimization},
volume = {26},
number = {3},
pages = {1835-1854},
year = {2016},
doi = {10.1137/130943170},

URL = { 
        https://doi.org/10.1137/130943170
    
},
eprint = { 
        https://doi.org/10.1137/130943170
    
}

}

@ARTICLE{xiao, 
author={J. Xiao and A. Ribeiro and Z.Q. Luo and G. B. Giannakis}, 
journal={IEEE Signal Processing Magazine}, 
title={Distributed compression-estimation using wireless sensor networks}, 
year={2006}, 
volume={23}, 
number={4}, 
pages={27-41}, 
keywords={bandwidth allocation;data compression;mean square error methods;wireless sensor networks;bandwidth requirements;centralized clairvoyant estimators;distributed compression-estimation;information theoretic perspective;mean square error;rate-constrained distributed estimators;signal processing algorithms;wireless sensor networks;Algorithm design and analysis;Bandwidth;Batteries;Network topology;Robustness;Sensor phenomena and characterization;Signal design;Signal processing;Signal processing algorithms;Wireless sensor networks}, 
doi={10.1109/MSP.2006.1657815}, 
ISSN={1053-5888}, 
month={July},}

@ARTICLE{learning, 
author={A. Nedi\'{c} and A. Olshevsky and C. A. Uribe}, 
journal={IEEE Transactions on Automatic Control}, 
title={Fast Convergence Rates for Distributed Non-Bayesian Learning}, 
year={2017}, 
volume={62}, 
number={11}, 
pages={5538-5553}, 
keywords={Bayes methods;convergence;distributed algorithms;learning (artificial intelligence);network theory (graphs);random processes;statistical distributions;conditionally independent random processes;distributed algorithm;distributed nonbayesian learning;distributed observations;explicit convergence rate;fast convergence rates;geometric convergence rate;improved learning protocol;nonasymptotic convergence rate;static networks;Bayes methods;Convergence;Estimation;Probability distribution;Protocols;Random variables;Silicon;Algorithm design and analysis;Bayes methods;distributed algorithms;estimation;learning}, 
doi={10.1109/TAC.2017.2690401}, 
ISSN={0018-9286}, 
month={Nov},}

@INPROCEEDINGS{formation, 
author={R. L. Raffard and C. J. Tomlin and S. P. Boyd}, 
booktitle={2004 43rd IEEE Conference on Decision and Control (CDC)}, 
title={Distributed optimization for cooperative agents: application to formation flight}, 
year={2004}, 
volume={3}, 
number={}, 
pages={2453-2459 Vol.3}, 
keywords={aerospace control;computational complexity;cooperative systems;multivariable systems;optimisation;artificially decomposed version;computationally intractable problem;convex examples;cooperative agents;decentralized algorithm;distributed optimization;dual decomposition techniques;formation flight;global optimum;nonconvex examples;optimization problems;Control systems;Distributed control;Iterative algorithms;Large-scale systems;Power system control;Power system stability;Power systems;Sensor systems;Upper bound;Vehicles}, 
doi={10.1109/CDC.2004.1428778}, 
ISSN={0191-2216}, 
month={Dec},}

@article{admm,
url = {http://dx.doi.org/10.1561/2200000016},
year = {2011},
volume = {3},
journal = {Foundations and Trends® in Machine Learning},
title = {Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers},
doi = {10.1561/2200000016},
issn = {1935-8237},
number = {1},
pages = {1-122},
author = {S. Boyd and N. Parikh and E. Chu and B. Peleato and J. Eckstein}
}

@ARTICLE{harnessing, 
author={G. Qu and N. Li}, 
journal={IEEE Transactions on Control of Network Systems}, 
title={Harnessing Smoothness to Accelerate Distributed Optimization}, 
year={2017}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Algorithm design and analysis;Control systems;Convergence;Distributed algorithms;Estimation;History;Optimization}, 
doi={10.1109/TCNS.2017.2698261}, 
ISSN={2325-5870}, 
month={},}

@ARTICLE{application,
author={I. Neocara and V. Nedelcu and Ioan Dumitrache},
journal={Journal of Process Control},
title={Parallel and distributed optimization methods for estimation and control in networks},
year={2011},
volume = {21},
number = {5},
pages = {756-766},
ISSN={0959-1524},
keywords={Estimation;Cooperative and distributed control;Networks of interconnected subsystems;
Convex optimization;Parallel and distributed methods;Duality theory;Consensus},
}



@ARTICLE{nedic, 
author={A. Nedi\'{c} and A. Ozdaglar}, 
journal={IEEE Transactions on Automatic Control}, 
title={Distributed Subgradient Methods for Multi-Agent Optimization}, 
year={2009}, 
volume={54}, 
number={1}, 
pages={48-61}, 
keywords={convex programming;distributed processing;gradient methods;minimisation;multi-agent systems;convex optimization;distributed computation model;distributed subgradient methods;multiagent optimization;time-varying topology;Character generation;Computational modeling;Convergence;Cost function;Distributed computing;Distributed control;Large-scale systems;Network topology;Optimization methods;Resource management;Convex optimization;cooperative control;distributed optimization;multi-agent network;subgradient method}, 
doi={10.1109/TAC.2008.2009515}, 
ISSN={0018-9286}, 
month={Jan},}

@ARTICLE{giannakis, 
author={G. B. Giannakis and V. Kekatos and N. Gatsis and S. J. Kim and H. Zhu and B. F. Wollenberg}, 
journal={IEEE Signal Processing Magazine}, 
title={Monitoring and Optimization for Power Grids: A Signal Processing Perspective}, 
year={2013}, 
volume={30}, 
number={5}, 
pages={107-128}, 
keywords={optimisation;power grids;power markets;power supply quality;power system interconnection;power system measurement;power system security;power system stability;power system state estimation;renewable energy sources;20th century;North American power grid;business opportunities;cascade failures;complex interconnections;consumer participation;cyberattacks;digital technology;environmental incentives;grid efficiency;grid operation;intelligent grid infrastructure;power grid monitoring;power grid optimization;renewable energy resources;Integrated circuit modeling;Load flow;Mathematical model;Power distribution;Power grids;State estimation}, 
doi={10.1109/MSP.2013.2245726}, 
ISSN={1053-5888}, 
month={Sept},}

@ARTICLE{estimation, 
author={I. D. Schizas and A. Ribeiro and G. B. Giannakis}, 
journal={IEEE Transactions on Signal Processing}, 
title={Consensus in Ad Hoc {WSN}s With Noisy Links 2014;Part I: Distributed Estimation of Deterministic Signals}, 
year={2008}, 
volume={56}, 
number={1}, 
pages={350-364}, 
keywords={ad hoc networks;least squares approximations;quantisation (signal);wireless sensor networks;ad hoc WSN;best linear unbiased estimation;block coordinate descent approach;decentralized algorithm;deterministic signal estimation;distributed estimation algorithm;least-squares estimation;multiplier method;noisy link;quantization noise;wireless sensor network;Bandwidth;Constraint optimization;Convergence;Data models;Maximum likelihood estimation;Quantization;Resilience;Robustness;Sensor fusion;Wireless sensor networks;Distributed estimation;nonlinear optimization;wireless sensor networks (WSNs)}, 
doi={10.1109/TSP.2007.906734}, 
ISSN={1053-587X}, 
month={Jan},}

@ARTICLE{next, 
author={P. D. Lorenzo and G. Scutari}, 
journal={IEEE Transactions on Signal and Information Processing over Networks}, 
title={{NEXT}: In-Network Nonconvex Optimization}, 
year={2016}, 
volume={2}, 
number={2}, 
pages={120-136}, 
keywords={approximation theory;concave programming;convex programming;minimisation;multi-agent systems;agent sum-utility;algorithmic framework;asymptotic convergence;convex approximation techniques;convex regularizer;distributed minimization;dynamic consensus mechanism;in-network nonconvex optimization;multi-agent networks;nonconvex distributed optimization;time-varying connectivity;Algorithm design and analysis;Approximation algorithms;Convergence;Heuristic algorithms;Information processing;Optimization;Signal processing algorithms;Consensus;distributed optimization;nonconvex optimization;successive convex approximation;time-varying directed graphs}, 
doi={10.1109/TSIPN.2016.2524588}, 
ISSN={2373-776X}, 
month={June},}

@INPROCEEDINGS{localization, 
author={M. G. Rabbat and R. D. Nowak}, 
booktitle={2004 IEEE International Conference on Acoustics, Speech, and Signal Processing}, 
title={Decentralized source localization and tracking [wireless sensor networks]}, 
year={2004}, 
volume={3}, 
number={},  
keywords={convergence of numerical methods;gradient methods;position measurement;sensor fusion;target tracking;wireless sensor networks;bandwidth requirements;collaborative signal processing;convergence rate theory;data fusion;decentralized source localization;energy requirements;gradient descent algorithm;in-network communication;incremental subgradient optimization methods;network size effects;received signal strength measurements;source location accurate estimate;source tracking;wireless sensor networks;Bandwidth;Collaboration;Collaborative work;Optimization methods;Position measurement;Robustness;Routing;Signal processing algorithms;Target tracking;Wireless sensor networks}, 
doi={10.1109/ICASSP.2004.1326696}, 
ISSN={1520-6149}, 
month={May},}

@ARTICLE{tutorial, 
author={D. P. Palomar and M. Chiang}, 
journal={IEEE Journal on Selected Areas in Communications}, 
title={A tutorial on decomposition methods for network utility maximization}, 
year={2006}, 
volume={24}, 
number={8}, 
pages={1439-1451}, 
keywords={distributed algorithms;gradient methods;radio networks;resource allocation;Gauss-Seidel iteration;Jacobi method;Lagrange duality;decomposition method;decoupling technique;distributed algorithm;modular network;network utility maximization;resource allocation;subgradient method;Congestion control;cross-layer design;decomposition;distributed algorithm;network architecture;network control by pricing;network utility maximization;optimization;power control;resource allocation}, 
doi={10.1109/JSAC.2006.879350}, 
ISSN={0733-8716}, 
month={Aug},}


@article{extra,
author = {W. Shi and Q. Ling and Gang Wu and W. Yin},
title = {EXTRA: An Exact First-Order Algorithm for Decentralized Consensus Optimization},
journal = {SIAM Journal on Optimization},
volume = {25},
number = {2},
pages = {944-966},
year = {2015},
doi = {10.1137/14096668X},

URL = { 
        https://doi.org/10.1137/14096668X
    
},
eprint = { 
        https://doi.org/10.1137/14096668X
    
}

}

@article{interpret,
author = {A. Nedi\'{c} and A. Olshevsky and W. Shi},
title = {Achieving Geometric Convergence for Distributed Optimization Over Time-Varying Graphs},
journal = {SIAM Journal on Optimization},
volume = {27},
number = {4},
pages = {2597-2633},
year = {2017},
doi = {10.1137/16M1084316},

URL = { 
        https://doi.org/10.1137/16M1084316
    
},
eprint = { 
        https://doi.org/10.1137/16M1084316
    
}

}

@ARTICLE{pextra, 
author={W. Shi and Q. Ling and G. Wu and W. Yin}, 
journal={IEEE Transactions on Signal Processing}, 
title={A Proximal Gradient Algorithm for Decentralized Composite Optimization}, 
year={2015}, 
volume={63}, 
number={22}, 
pages={6013-6023}, 
keywords={compressed sensing;convergence;gradient methods;learning (artificial intelligence);multi-agent systems;quadratic programming;Lipschitz gradients;P-EXTRA;PG-EXTRA;compressed sensing problems;consensus minimizer;consensus optimization problem;decentralized composite optimization;decentralized constrained quadratic programming;ergodic convergence rate;first-order optimality residual;fixed step size;inverse problems;local objective functions;machine learning;proximal gradient algorithm;proximal gradient exact first-order algorithm;signal processing;smooth+nonsmooth composite form;static networked multiagent system;Compressed sensing;Convergence;Linear programming;Optimization;Signal processing;Signal processing algorithms;Symmetric matrices;Composite objective;decentralized optimization;multi-agent network;nonsmooth;proximal;regularization}, 
doi={10.1109/TSP.2015.2461520}, 
ISSN={1053-587X}, 
month={Nov},}

@misc{optimal,
author = {K. Scaman and F. Back and S. Bubeck and Y. T. Lee and L. Massouli\'{e}},
title ={Optimal algorithms for smooth and strongly convex distributed optimization in networks},
year = {2017},
howpublished={arXiv: 1702.08704},
}

@ARTICLE{random_networks, 
author={M. Hong and T. H. Chang}, 
journal={IEEE Transactions on Signal Processing}, 
title={Stochastic Proximal Gradient Consensus Over Random Networks}, 
year={2017}, 
volume={65}, 
number={11}, 
pages={2933-2948}, 
keywords={convex programming;distributed algorithms;iterative methods;network theory (graphs);stochastic processes;convex optimization problem;distributed algorithm;dynamic stochastic proximal-gradient consensus algorithm;iteration counter;random network;randomly time-varying multiagent network;randomly time-varying network;stochastic proximal gradient consensus;Algorithm design and analysis;Convergence;Convex functions;Heuristic algorithms;Linear programming;Optimization;Signal processing algorithms;ADMM;Distributed optimization;fast algorithms;rate analysis}, 
doi={10.1109/TSP.2017.2673815}, 
ISSN={1053-587X}, 
month={June},}

@ARTICLE{time_varying_graphs, 
author={A. Nedić and A. Olshevsky}, 
journal={IEEE Transactions on Automatic Control}, 
title={Distributed Optimization Over Time-Varying Directed Graphs}, 
year={2015}, 
volume={60}, 
number={3}, 
pages={601-615}, 
keywords={directed graphs;optimisation;time-varying systems;broadcast-based algorithm;convex function;distributed optimization;graph sequence;network information diffusion;proportionality constant;subgradient boundedness;subgradient-push;time-varying directed graphs;time-varying sequence;Convergence;Convex functions;Equations;Optimization;Protocols;Standards;Vectors;Time-varying;UAVs}, 
doi={10.1109/TAC.2014.2364096}, 
ISSN={0018-9286}, 
month={March},}

@ARTICLE{subgradient, 
author={A. Nedi\'{c} and A. Ozdaglar}, 
journal={IEEE Transactions on Automatic Control}, 
title={Distributed Subgradient Methods for Multi-Agent Optimization}, 
year={2009}, 
volume={54}, 
number={1}, 
pages={48-61}, 
keywords={convex programming;distributed processing;gradient methods;minimisation;multi-agent systems;convex optimization;distributed computation model;distributed subgradient methods;multiagent optimization;time-varying topology;Character generation;Computational modeling;Convergence;Cost function;Distributed computing;Distributed control;Large-scale systems;Network topology;Optimization methods;Resource management;Convex optimization;cooperative control;distributed optimization;multi-agent network;subgradient method}, 
doi={10.1109/TAC.2008.2009515}, 
ISSN={0018-9286}, 
month={Jan},}

@inproceedings{dual_decomposition,
author = {H. Terelius and U. Topcu and R. M. Murray},
booktitle={2011 IFAC Proceedings}, 
title={Decentralized Multi-Agent Optimization via Dual Decomposition}, 
year={2011}, 
volume={44}, 
number={}, 
pages={11245-11251 vol.1},  
ISSN={1474-6670}, }

@INPROCEEDINGS{non_convex, 
author={Y. Sun and G. Scutari and D. Palomar}, 
booktitle={2016 50th Asilomar Conference on Signals, Systems and Computers}, 
title={Distributed nonconvex multiagent optimization over time-varying networks}, 
year={2016}, 
volume={}, 
number={}, 
pages={788-794}, 
keywords={concave programming;directed graphs;information dissemination;minimisation;multi-agent systems;network theory (graphs);time-varying networks;SCA;agent cost functions;agent sum-utility;arbitrary time-varying digraphs;asymptotic convergence;broadcast protocol;broadcast-based distributed algorithm;broadcast-based distributed algorithmic framework;consensus matrices;convex constrained optimization;distributed nonconvex multiagent optimization;graph sequence knowledge;hinges;information dissemination;multiagent networks;node communications;nonconvex function;nonseparable function;successive convex approximation;time-varying networks;time-varying sequence;Algorithm design and analysis;Convergence;Cost function;Distributed algorithms;Network topology;Protocols}, 
doi={10.1109/ACSSC.2016.7869154}, 
ISSN={}, 
month={Nov},}

@techreport{oracle,
title={First-order methods with inexact oracle: the strongly convex case},
author={O. Devolder and F. Glineur and Y. Nesterov},
year = {2013},
institution={UCL},
year={2013},
}

@book{nesterov,
author = {Yuri Nesterov},
title = {Introductory Lectures on Convex Optimization: A Basic Course},
publisher = {Springer-Verlag US},
year = {2004},

}

@book{rockafellar,
author = {R. Tyrell Rockafellar},
title = {Convex Analysis},
publisher= {Princeton University Press},
year = {1970},
}

@article{luo,
author = {Zhi-Quan Luo and Paul Tseng},
title = {On the Convergence Rate of Dual Ascent Methods for Linearly Constrained Convex Minimization},
journal = {Mathematics of Operations Research},
volume = {18},
number = {4},
pages = {846-867},
year = {1993},
doi = {10.1287/moor.18.4.846},

URL = { 
        https://doi.org/10.1287/moor.18.4.846
    
},
eprint = { 
        https://doi.org/10.1287/moor.18.4.846
    
}
,
    abstract = { We analyze the rate of convergence of certain dual ascent methods for the problem of minimizing a strictly convex essentially smooth function subject to linear constraints. Included in our study are dual coordinate ascent methods and dual gradient methods. We show that, under mild assumptions on the problem, these methods attain a linear rate of convergence. Our proof is based on estimating the distance from a feasible dual solution to the optimal dual solution set by the norm of a certain residual. }
}

@article{non-strongly,
abstract = {The standard assumption for proving linear convergence of first order methods for smooth convex optimization is the strong convexity of the objective function, an assumption which does not hold for many practical applications. In this paper, we derive linear convergence rates of several first order methods for solving smooth non-strongly convex constrained optimization problems, i.e. involving an objective function with a Lipschitz continuous gradient that satisfies some relaxed strong convexity condition. In particular, in the case of smooth constrained convex optimization, we provide several relaxations of the strong convexity conditions and prove that they are sufficient for getting linear convergence for several first order methods such as projected gradient, fast gradient and feasible descent methods. We also provide examples of functional classes that satisfy our proposed relaxations of strong convexity conditions. Finally, we show that the proposed relaxed strong convexity conditions cover important applications ranging from solving linear systems, Linear Programming, and dual formulations of linearly constrained convex problems.},
author = {Necoara, I and Nesterov, Yu. and Glineur, F},
doi = {10.1007/s10107-018-1232-1},
issn = {1436-4646},
journal = {Mathematical Programming},
month = {jan},
title = {{Linear convergence of first order methods for non-strongly convex optimization}},
url = {https://doi.org/10.1007/s10107-018-1232-1},
year = {2018}
}
@inproceedings{polyak,
abstract = {In 1963, Polyak proposed a simple condition that is sufficient to show a global linear convergence rate for gradient descent. This condition is a special case of the {\L}ojasiewicz inequality proposed in the same year, and it does not require strong convexity (or even convexity). In this work, we show that this much-older Polyak-{\L}ojasiewicz (PL) inequality is actually weaker than the main conditions that have been explored to show linear convergence rates without strong convexity over the last 25 years. We also use the PL inequality to give new analyses of coordinate descent and stochastic gradient for many non-strongly-convex (and some non-convex) functions. We further propose a generalization that applies to proximal-gradient methods for non-smooth optimization, leading to simple proofs of linear convergence for support vector machines and L1-regularized least squares without additional assumptions.},
address = {Cham},
author = {Karimi, Hamed and Nutini, Julie and Schmidt, Mark},
booktitle = {Machine Learning and Knowledge Discovery in Databases},
editor = {Frasconi, Paolo and Landwehr, Niels and Manco, Giuseppe and Vreeken, Jilles},
isbn = {978-3-319-46128-1},
pages = {795--811},
publisher = {Springer International Publishing},
title = {{Linear Convergence of Gradient and Proximal-Gradient Methods Under the Polyak-{\L}ojasiewicz Condition}},
year = {2016}
}

@misc{maros,
author={M. Maros and J. Jald\'{e}n},
title = {On the {Q}-linear convergence of Distributed Generalized {ADMM} under non-strongly convex
function components},
year = {2018},
howpublished = {arXiv: 1805.01660}
}

@article{martinez,
author={M. Zhu and S. Martinez},
title={Discrete-Time Dynamic Average Consensus},
journal={Automatica},
volume = {46},
number = {2},
pages = {322-329},
year = {2010}
}

@ARTICLE{dadmm, 
author={W. Shi and Q. Ling and K. Yuan and G. Wu and W. Yin}, 
journal={IEEE Transactions on Signal Processing}, 
title={On the Linear Convergence of the {ADMM} in Decentralized Consensus Optimization}, 
year={2014}, 
volume={62}, 
number={7}, 
pages={1750-1761}, 
keywords={convergence;convex programming;iterative methods;multi-agent systems;ADMM convergence;alternating direction method of multipliers;common decision variable;convex local objective functions;decentralized consensus optimization;information exchange;iterative computation method;linear convergence;theoretical convergence rate;Convergence;Convex functions;Information exchange;Linear programming;Optimization;Signal processing algorithms;Vectors;Decentralized consensus optimization;alter nating direction method of multipliers (ADMM);linear convergence}, 
doi={10.1109/TSP.2014.2304432}, 
ISSN={1053-587X}, 
month={April},}

@ARTICLE{dlm, 
author={Q. Ling and W. Shi and G. Wu and A. Ribeiro}, 
journal={IEEE Transactions on Signal Processing}, 
title={{DLM}: Decentralized Linearized Alternating Direction Method of Multipliers}, 
year={2015}, 
volume={63}, 
number={15}, 
pages={4051-4064}, 
keywords={gradient methods;least mean squares methods;multi-agent systems;optimisation;regression analysis;signal processing;Lipschitz continuous gradients;decentralized linearized alternating direction method of multipliers;distributed gradient method;gradient descent step;least squares;local cost functions;logistic regression problems;multiagent network;Convergence;Cost function;Eigenvalues and eigenfunctions;Gradient methods;Minimization;Signal processing algorithms;Decentralized optimization;linearized alternating direction method of multipliers;multiagent network}, 
doi={10.1109/TSP.2015.2436358}, 
ISSN={1053-587X}, 
month={Aug},}

@ARTICLE{harnesing, 
author={G. Qu and N. Li}, 
journal={IEEE Transactions on Control of Network Systems}, 
title={Harnessing Smoothness to Accelerate Distributed Optimization}, 
year={2017},  
pages={To appear}, 
keywords={Algorithm design and analysis;Control systems;Convergence;Distributed algorithms;Estimation;History;Optimization}, 
doi={10.1109/TCNS.2017.2698261}, 
ISSN={2325-5870}, 
month={},}

@incollection{learning2,
author = {G. Giannakis and Q. Ling and G. Mateos and I.D. Schizas and H. Zhu},
title = {Decentralized Learning for Wireless Communications and Networking},
editor = {R. Glowinski and S. Osher and W. Yin},
booktitle = {Splitting methods in Communication, Imaging, Science and Engineering},
pages = {461-467},
publisher = {Springer, Cham},
year = {2016},
}

@article{social_learning,
author = {A. Jadbabaie and P. Molavi and A. Sandroni and A. Tahbaz-Salehi},
title = {Non-Bayesian social learning},
journal = {Games and Economic Behavior},
volume = {76},
number = {1},
year = {2012},
pages = {210-225},
}

@INPROCEEDINGS{unc_step, 
author={A. Nedi\'{c} and A. Olshevsky and W. Shi and C. A. Uribe}, 
booktitle={2017 American Control Conference (ACC)}, 
title={Geometrically convergent distributed optimization with uncoordinated step-sizes}, 
year={2017}, 
volume={}, 
number={}, 
pages={3950-3955}, 
keywords={convergence;geometry;graph theory;optimisation;ATC structure;ATC variation;Adapt-Then-Combine variation;DGD structure;DIGing algorithm;algorithmic family;convergent distributed optimization;distributed gradient descent;geometric convergence;time-varying undirected/directed graphs;uncoordinated step-sizes;Algorithm design and analysis;Convergence;Convex functions;Inference algorithms;Linear programming;Optimization;Radio frequency}, 
doi={10.23919/ACC.2017.7963560}, 
ISSN={}, 
month={May},}

@misc{frost,
author = {R. Xin and C. Xi and U.A. Khan},
title ={{FROST}-Fast row-stochastic optimization with uncoordinated step-sizes},
year = {2018},
howpublished={arXiv: 1803.09169},
}

@misc{addopt,
author = {C.Xi and R. Xin and U.A. Khan},
title = {{ADD-OPT}: Accelerated Distributed Directed optimization},
year = {2017},
howpublished = {arXiv: 1607.04757},
}

@misc{panda,
author= {M. Maros and J. Jald\'{e}n},
title = {PANDA: A Dual Linearly Converging Method for Distributed Optimization over Time Varying Graphs},
year = {2018},
howpublished = {arXiv: 1803.0328v2}}
@ARTICLE{dextra, 
author={C. Xi and U. A. Khan}, 
journal={IEEE Transactions on Automatic Control}, 
title={{DEXTRA}: A Fast Algorithm for Optimization Over Directed Graphs}, 
year={2017}, 
volume={62}, 
number={10}, 
pages={4980-4993}, 
keywords={convergence;convex programming;distributed algorithms;iterative methods;mathematics computing;DEXTRA;agents;convergence rates;directed graphs;distributed algorithm;general convex objective functions;iterations;local objective functions;optimization problem;Acceleration;Convergence;Distributed algorithms;Indexes;Linear programming;Optimization;Symmetric matrices;Directed graphs;distributed optimization;multiagent networks}, 
doi={10.1109/TAC.2017.2672698}, 
ISSN={0018-9286}, 
month={Oct},}

@misc{fenchel,
author = {X. Wu and J. Lu},
title = {Fenchel Dual Gradient Methods for Distributed Convex Optimization over Time-Varying Networks},
year = {2017},
howpublished = {arXiv: 1708.07620},
}

@ARTICLE{grid, 
author={T. Yang and J. Lu and D. Wu and J. Wu and G. Shi and Z. Meng and K. H. Johansson}, 
journal={IEEE Transactions on Industrial Electronics}, 
title={A Distributed Algorithm for Economic Dispatch Over Time-Varying Directed Networks With Delays}, 
year={2017}, 
volume={64}, 
number={6}, 
pages={5095-5106}, 
keywords={cost reduction;power generation dispatch;power generation economics;EDP;bounded time-varying delays;communication delays;communication links;distributed algorithm;economic dispatch problem;generator capacity limits;gradient push-sum method;numerical simulation;power system operation;time-varying directed communication network;time-varying topology;total generation cost minimization;Communication networks;Cost function;Delay effects;Delays;Distributed algorithms;Generators;Network topology;Distributed algorithm;economic dispatch;gradient push-sum method;time-varying delays;time-varying networks}, 
doi={10.1109/TIE.2016.2617832}, 
ISSN={0278-0046}, 
month={June},}
@misc{toyota,
title= {On the duality of strong convexity and strong smoothness: Learning applications and matrix regulation},
year={2009},
author={S.M. Kadade and S.Shalev-Shwarz, A. Tweari},
howpublished={Technical Report, Toyota Technological Insitute, Chicago-USA},
}
@misc{time_nesterov,
author = {A. Rogozin and C.A. Uribe and A. Gasnikov and N. Malkovsky and A. Nedi\'{c}},
title ={Optimal distributed convex optimization on slowly time-varying graphs},
year = {2018},
howpublished={arXiv: 1805.06045v1},
}


\bibitem{xiao}
J.J~.Xiao, A.~Ribeiro, et. al. ``Distributed compression-estimation using wireless sensor networks," \emph{IEEE Signal Proc. Magazine,} vol. 23, no. 4, pp. 27-41, July 2006.
\bibitem{decentralized_gradient}
K.~Yuan, Q.~Ling, et. al. ``On the Convergence of Decentralized Gradient Descent," \emph{SIAM. J. Optim.,} vol. 26, no. 3, pp. 1835-1854, September 2016.
\bibitem{learning}
A.~Nedi\'{c}, A.~Olshvesky, et. al. ``Fast Convergence Rates for Distributed Non-Bayesian Learning," \emph{IEEE Trans. Autom. Control,} vol. 62, no. 11, pp. 5538-553, March 2017.
\bibitem{learning2}
G.~Giannakis, Q.~Ling, et. al. ``Decentralized Learning for Wireless Communications and Networking." In: R.~Glowinski, S.~Osher, et. al. (eds) ``Splitting Methods in Communication, Imaging, Science and Engineering," Scientific Computation. Springer, Cham. 
\bibitem{formation}
R.L.~Raffard, C.J.~Tomlin, et. al. ``Optimization for Cooperative Agents: Application to Formation Flight," \emph{The 43rd IEEE Annual Conference on Decision and Control,} 2004, pp. 2453-2459.
\bibitem{admm}
S.~Boyd, N.~Parikh, et. al., ``Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers," \emph{Foundation and Trends\textregistered in Machine Learning,} vol. 3, no. 1, pp.1-122, January 2011.
\bibitem{harnesing}
G.~Qu, N.~Li, ``Harnessing Smoothness to Accelerate Distributed Optimization," \emph{IEEE Trans. Autom. Control,} to appear.
\bibitem{application}
I.~Necoara, V.~Nedelcu, et. al., ``Parallel and distributed optimization methods for estimation and control in networks," \emph{Journal of Process Control,} vol. 21, no. 5, pp. 756-766, June 2011. 
\bibitem{nedic}
A.~Nedi\'{c}, A~Ozdaglar, ``Distributed Subgradient Methods for Multi-Agent Optimization," \emph{IEEE Trans. Autom. Control,} vol. 54, no. 1, pp. 48-60, January 2009.
\bibitem{giannakis}
G.B.~Giannakis, V.~Kekatos, et. al. ``Monitoring and Optimization for Power Grids: A Signal Processing Perspective," \emph{IEEE Signal Process. Magazine,} vol. 30, no. 5, pp. 107-128, August 2013.
\bibitem{estimation}
I.D.~Schizas, A.~Ribeiro, et. al. ``Consensus in Ad Hoc WSNs with Noisy Links-Part 1: Distributed Estimation of Deterministic Signals," \emph{IEEE Trans. Signal Process.,} vol. 56, no. 1, pp. 350-364, December 2007.
\bibitem{next}
P.~Lorenzo, G.~Scutari, ``NEXT: In-Network Nonconvex Optimization," \emph{IEEE Trans. Signal and Info. Proc. over Networks.} vol. 2, no. 2, pp. 120-136, June 2016.
\bibitem{localization}
M.G.~Rabbat, R.D.~Nowak, ``Decentralized source localization and tracking [wireless sensor networks]," \emph{Proc. IEEE ICASSP,} May 2004.
\bibitem{tutorial}
D.P.~Palomar, M~Chaing, ``A tutorial on decomposition methods for network utility maximization," \emph{IEEE Journal on Selected Areas in Communications,} vol. 8, no. 1, pp. 1439-1451, August 2006.
\bibitem{extra}
W.~Shi, Q.~Ling, et. al., ``EXTRA: An Exact First-Order Algorithm for Decentralized Consensus Optimization," \emph{SIAM J. Optim.,} vol. 25, no. 5, pp. 944-966, May 2015.
\bibitem{interpret}
A.~Nedi\'{c}, A.~Olshevsky, et. al., ``Achieving Geometric Convergence for Distributed Optimization Over Time-Varying Graphs," \texttt{arxiv:1607.03218v3}, March 2017.
\bibitem{pextra}
W.~Shi, Q.~Ling, et. al. ``A Proximal Gradient Algorithm for Decentralized Composite Optimization," \emph{IEEE Trans. Signal Process.,} vol. 63, no. 22, pp. 6013-6023, November 2015.
\bibitem{optimal}
K.~Scaman, F.~Back, et. al. ``Optimal algorithms for smooth and strongly convex distributed optimization in networks," \texttt{arxiv:1702.08704v2,} April 2017.
\bibitem{random_networks}
M.~Hong, T.~Chang, ``Stochastic Proximal Gradient Consensus over Random Networks," \emph{IEEE Trans. Signal Process.,} vol. 65, no. 11, pp. 2933-2948, June 2017.
\bibitem{time_varying_graphs}
A.~Nedi\'{c}, A.~Olshevsky, ``Distributed optimization over time-varying directed graphs," \emph{IEEE Trans. Automat. Control,} vol 60, no. 3, pp. 601-615, October 2014.
\bibitem{subgradient}
A.~Nedi\'{c} and A.~Ozdaglar, ``Distributed Subgradient Method for Multi-agent Optimization," \emph{IEEE Trans. Automat. Control,} vol 54, no. 1, pp. 48-61, January 2009.
\bibitem{dual_decomposition}
H.~Terelius, U.~Topcu, et. al, ``Decentralized multi-agent optimization via dual decomposition," \emph{Proc. IFAC,} vol. 44, no. 1, pp. 11245-11251, January 2011.
\bibitem{non_convex}
Y.~Sun, G.~Scutari, et. al. ``Distributed nonconvex Multiagent optimization Over Time-Varying networks," \emph{Asilomar}, March 2017.
\bibitem{oracle}
O.~Devolder, F.~Glineur, et. al. ``First-order methods with inexact oracle: the strongly convex case," \emph{Tech. report, UCL}, 2013.
\bibitem{dual_smooth}
S.~Kakade, S.~Shalev-Shwartz, et. al. ``On the duality of strong convexity and strong smoothness: Learning applications and matrix regularization," 2009.
\bibitem{nesterov}
Y.~Nesterov, ``Introductory lectures on Convex Optimization: A Basic Course," Springer-Verlag, US, 2004.
\bibitem{luo}
Z.Q.~Luo, P.~Tseng, ``On the Convergence Rate of Dual Ascent Methods for Linearly Constrained Convex Minimization," \emph{Math. Oper. Res.,} vol. 18, no. 4, pp. 846-867, 1993.
\bibitem{martinez}
M.~Zhu, S.~Martinez, ``Discrete-Time Dynamic Average Consensus," \emph{Automatica,} vol. 46, no. 2, pp. 322-329, 2010.
\bibitem{dadmm}
W.~Shi, Q.~Ling, et. al. ``On the Linear Convergence of the ADMM in Decentralized Consensus Optimization,"\emph{IEEE Trans. on Signal Process.,} vol. 46, no. 7, April 2014.
\bibitem{dlm}
Q.~Ling, W.~Shi, et. al. ``DLM: Decentralized linearized alternating direction method of multipliers," \emph{IEEE Trans. on Signal Process.,} vol. 63, no. 15, August 2015.
